The Search for Sparse, Robust Neural Networks

Recent work on deep neural network pruning has shown there exist sparse subnetworks that achieve equal or improved accuracy, training time, and loss using fewer network parameters when compared to their dense counterparts. Orthogonal to pruning literature, deep neural networks are known to be susceptible to adversarial examples, which may pose risks in security- or safety-critical applications. Intuition suggests that there is an inherent trade-off between sparsity and robustness such that these characteristics could not co-exist. We perform an extensive empirical evaluation and analysis testing the Lottery Ticket Hypothesis with adversarial training and show this approach enables us to find sparse, robust neural networks. Code for reproducing experiments is available here: https://github.com/justincosentino/robust-sparse-networks.

==> __latexindent_temp.tex <==
@article{liu2018rethinking,
  title={Rethinking the value of network pruning},
  author={Liu, Zhuang and Sun, Mingjie and Zhou, Tinghui and Huang, Gao and Darrell, Trevor},
  journal={arXiv preprint arXiv:1810.05270},
  year={2018}
}

@article{frankle2018lottery,
  title={The lottery ticket hypothesis: Finding sparse, trainable neural networks},
  author={Frankle, Jonathan and Carbin, Michael},
  journal={arXiv preprint arXiv:1803.03635},
  year={2018}
}

@article{goodfellow2014explaining,
  title={Explaining and harnessing adversarial examples},
  author={Goodfellow, Ian J and Shlens, Jonathon and Szegedy, Christian},
  journal={arXiv preprint arXiv:1412.6572},
  year={2014}
}

@article{tsipras2018robustness,
  title={Robustness may be at odds with accuracy},
  author={Tsipras, Dimitris and Santurkar, Shibani and Engstrom, Logan and Turner, Alexander and Madry, Aleksander},
  journal={stat},
  volume={1050},
  pages={11},
  year={2018}
}

@article{madry2017towards,
  title={Towards deep learning models resistant to adversarial attacks},
  author={Madry, Aleksander and Makelov, Aleksandar and Schmidt, Ludwig and Tsipras, Dimitris and Vladu, Adrian},
  journal={arXiv preprint arXiv:1706.06083},
  year={2017}
}

@article{wong2017provable,
  title={Provable defenses against adversarial examples via the convex outer adversarial polytope},
  author={Wong, Eric and Kolter, J Zico},
  journal={arXiv preprint arXiv:1711.00851},
  year={2017}
}

@article{sinha2017certifiable,
  title={Certifiable distributional robustness with principled adversarial training},
  author={Sinha, Aman and Namkoong, Hongseok and Duchi, John},
  journal={stat},
  volume={1050},
  pages={29},
  year={2017}
}

@article{raghunathan2018certified,
  title={Certified defenses against adversarial examples},
  author={Raghunathan, Aditi and Steinhardt, Jacob and Liang, Percy},
  journal={arXiv preprint arXiv:1801.09344},
  year={2018}
}

@article{wang2018adversarial,
  title={Adversarial robustness of pruned neural networks},
  author={Wang, Luyu and Ding, Gavin Weiguang and Huang, Ruitong and Cao, Yanshuai and Lui, Yik Chau},
  year={2018}
}

@misc{xiao2017fashion,
  author={Han Xiao and Kashif Rasul and Roland Vollgraf},
  title={Fashion-MNIST: a Novel Image Dataset for Benchmarking Machine Learning Algorithms},
  date={2017-08-28},
  year={2017},
  eprintclass={cs.LG},
  eprinttype={arXiv},
  eprin={cs.LG/1708.07747},
}

@techreport{krizhevsky2009learning,
  title={Learning multiple layers of features from tiny images},
  author={Krizhevsky, Alex and Hinton, Geoffrey},
  year={2009},
  institution={Citeseer}
}

@inproceedings{deng2009imagenet,
  title={Imagenet: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle={2009 IEEE conference on computer vision and pattern recognition},
  pages={248--255},
  year={2009},
  organization={Ieee}
}

@inproceedings{han2015learning,
  title={Learning both weights and connections for efficient neural network},
  author={Han, Song and Pool, Jeff and Tran, John and Dally, William},
  booktitle={Advances in neural information processing systems},
  pages={1135--1143},
  year={2015}
}

@article{li2016pruning,
  title={Pruning filters for efficient convnets},
  author={Li, Hao and Kadav, Asim and Durdanovic, Igor and Samet, Hanan and Graf, Hans Peter},
  journal={arXiv preprint arXiv:1608.08710},
  year={2016}
}

@article{lecun1998gradient,
  title={Gradient-based learning applied to document recognition},
  author={LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick and others},
  journal={Proceedings of the IEEE},
  volume={86},
  number={11},
  pages={2278--2324},
  year={1998},
  publisher={Taipei, Taiwan}
}

@article{see2016compression,
  title={Compression of neural machine translation models via pruning},
  author={See, Abigail and Luong, Minh-Thang and Manning, Christopher D},
  journal={arXiv preprint arXiv:1606.09274},
  year={2016}
}

@inproceedings{papernot2017practical,
  title={Practical black-box attacks against machine learning},
  author={Papernot, Nicolas and McDaniel, Patrick and Goodfellow, Ian and Jha, Somesh and Celik, Z Berkay and Swami, Ananthram},
  booktitle={Proceedings of the 2017 ACM on Asia conference on computer and communications security},
  pages={506--519},
  year={2017},
  organization={ACM}
}

@article{papernot2018cleverhans,
  title={Technical Report on the CleverHans v2.1.0 Adversarial Examples Library},
  author={Nicolas Papernot and Fartash Faghri and Nicholas Carlini and
  Ian Goodfellow and Reuben Feinman and Alexey Kurakin and Cihang Xie and
  Yash Sharma and Tom Brown and Aurko Roy and Alexander Matyasko and
  Vahid Behzadan and Karen Hambardzumyan and Zhishuai Zhang and
  Yi-Lin Juang and Zhi Li and Ryan Sheatsley and Abhibhav Garg and
  Jonathan Uesato and Willi Gierke and Yinpeng Dong and David Berthelot and
  Paul Hendricks and Jonas Rauber and Rujun Long},
  journal={arXiv preprint arXiv:1610.00768},
  year={2018}
}

@inproceedings{abadi2016tensorflow,
  title={Tensorflow: A system for large-scale machine learning},
  author={Abadi, Mart{\'\i}n and Barham, Paul and Chen, Jianmin and Chen, Zhifeng and Davis, Andy and Dean, Jeffrey and Devin, Matthieu and Ghemawat, Sanjay and Irving, Geoffrey and Isard, Michael and others},
  booktitle={12th {USENIX} Symposium on Operating Systems Design and Implementation ({OSDI} 16)},
  pages={265--283},
  year={2016}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@article{szegedy2013intriguing,
  title={Intriguing properties of neural networks},
  author={Szegedy, Christian and Zaremba, Wojciech and Sutskever, Ilya and Bruna, Joan and Erhan, Dumitru and Goodfellow, Ian and Fergus, Rob},
  journal={arXiv preprint arXiv:1312.6199},
  year={2013}
}

@inproceedings{papernot2016limitations,
  title={The limitations of deep learning in adversarial settings},
  author={Papernot, Nicolas and McDaniel, Patrick and Jha, Somesh and Fredrikson, Matt and Celik, Z Berkay and Swami, Ananthram},
  booktitle={2016 IEEE European Symposium on Security and Privacy (EuroS\&P)},
  pages={372--387},
  year={2016},
  organization={IEEE}
}

@inproceedings{carlini2017towards,
  title={Towards evaluating the robustness of neural networks},
  author={Carlini, Nicholas and Wagner, David},
  booktitle={2017 IEEE Symposium on Security and Privacy (SP)},
  pages={39--57},
  year={2017},
  organization={IEEE}
}

@article{kurakin2016adversarial,
  title={Adversarial machine learning at scale},
  author={Kurakin, Alexey and Goodfellow, Ian and Bengio, Samy},
  journal={arXiv preprint arXiv:1611.01236},
  year={2016}
}

@article{frankle2019lottery,
  title={The Lottery Ticket Hypothesis at Scale},
  author={Frankle, Jonathan and Dziugaite, Gintare Karolina and Roy, Daniel M and Carbin, Michael},
  journal={arXiv preprint arXiv:1903.01611},
  year={2019}
}

@inproceedings{lecun1990optimal,
  title={Optimal brain damage},
  author={LeCun, Yann and Denker, John S and Solla, Sara A},
  booktitle={Advances in neural information processing systems},
  pages={598--605},
  year={1990}
}

@article{xiao2018training,
  title={Training for faster adversarial robustness verification via inducing relu stability},
  author={Xiao, Kai Y and Tjeng, Vincent and Shafiullah, Nur Muhammad and Madry, Aleksander},
  journal={arXiv preprint arXiv:1809.03008},
  year={2018}
}

@article{Cheng2017ASO,
  title={A Survey of Model Compression and Acceleration for Deep Neural Networks},
  author={Yu Cheng and Duo Wang and Pan Zhou and Tao Zhang},
  journal={CoRR},
  year={2017},
  volume={abs/1710.09282}
}

